Learning compositionally through attentive guidance

While neural network models have been successfully applied to domains that require substantial generalisation skills, recent studies have implied that they struggle when solving the task they are trained on requires inferring its underlying compositional structure. In this paper, we introduce Attentive Guidance, a mechanism to direct a sequence to sequence model equipped with attention to find more compositional solutions. We test it on two tasks, devised precisely to assess the compositional capabilities of neural models, and we show that vanilla sequence to sequence models with attention overfit the training distribution, while the guided versions come up with compositional solutions that fit the training and testing distributions almost equally well. Moreover, the learned solutions generalise even in cases where the training and testing distributions strongly diverge. In this way, we demonstrate that sequence to sequence models are capable of finding compositional solutions without requiring extra components. These results helps to disentangle the causes for the lack of systematic compositionality in neural networks, which can in turn fuel future work.

==> acknowledgements.tex <==
\section*{Acknowledgements}

We thank Marco Baroni for inspiration and his valuable feedback, and Facebook AI Research for sponsoring this project.


==> attention_plots.tex <==
\section{Attention patterns}
Below we provide here more examples of attention plots for models trained with AG. Correct outputs are coloured green, whereas incorrect outputs are coloured red.

\begin{figure}[!ht]
    \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=0.9\linewidth, trim={33mm, 0mm, 10mm, 0mm}, clip]{figures/attn_plots_appendix/pre_heldout1.png}
    \caption{Pre-rnn: Heldout Tables}\label{fig:attn_heldout1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\linewidth}
   	\includegraphics[width=0.9\linewidth, trim={33mm, 0mm, 10mm, 0mm}, clip]{figures/attn_plots_appendix/pre_heldout2.png}
   	\caption{Pre-rnn: Heldout Tables}\label{fig:attn_heldout2}
    \end{subfigure}\\
    \begin{subfigure}{0.48\linewidth}
   	\includegraphics[width=0.9\linewidth, trim={33mm, 0mm, 10mm, 0mm}, clip]{figures/attn_plots_appendix/pre_new1.png}
   	\caption{Pre-rnn: New Compositions}\label{fig:new1}
    \hfill
    \end{subfigure}
    \begin{subfigure}{0.48\linewidth}
   	\includegraphics[width=0.9\linewidth, trim={33mm, 0mm, 13mm, 0mm}, clip]{figures/attn_plots_appendix/pre_new2.png}
   	\caption{Pre-rnn: New Compositions}\label{fig:new2}
    \end{subfigure}\\
    \begin{subfigure}{0.48\linewidth}
   	\includegraphics[width=0.9\linewidth, trim={33mm, 0mm, 10mm, 0mm}, clip]{figures/attn_plots_appendix/pre_longer1.png}
   	\caption{Pre-rnn: Composition of length 3}\label{fig:3length1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=0.9\linewidth, trim={33mm, 0mm, 10mm, 0mm}, clip]{figures/attn_plots_appendix/pre_longer2.png}
   	\caption{Pre-rnn: Composition of length 3}\label{fig:3length2}
    \end{subfigure}
 % \caption{Attention distributions for learned pre-rnn}\label{fig:all_data}
\end{figure}


==> attentive_guidance.tex <==
\subsection{Intuition}

Imagine teaching a child how to read.
Rather than giving her increasingly long sequences of words and letters (the input) and starting to vocalise them (the target), you guide her to the process.
You draw her attention by pointing at individual letters, tell her how to pronounce them, and show her how together they form a word.
That is, you inform her about the individual components of the task of reading, and you tell her how these can be (compositionally) combined.
Attentive guidance is based on exactly this idea: Via the attention component of a model, we explicitly tell the model how it should attend the input in a compositional way.
From an intuitive perspective, this can be interpreted as guiding the model through generating outputs following an appropriate protocol, by telling it what the different parts of the input are and when they should be attended.
More technically, guiding the attention vector of a model discourages \kris{I don't know if this is the "technical" explanation, and I don't know if the term 'discourage' is a behaviour we can back up with our results. We don't know why exactly our solution works, we only have an intuition} solutions that strongly rely on memorisation of spurious patterns and pushes them to develop and use representations for sensible subsequences instead. \dieuwke{Kris has a point here, the word 'technically' is a bit out of place somehow. Can we put in this intuition in another way? For instance by putting back in the example in comments?}

% For instance, a vanilla network might memorise the meaning of a phrase like `John loves Mary' as a whole, not allowing it to generalise to also understand `Mary love john', whereas an attention guided is stimulated to generate a separate reprentation for the word `love' on its own.\dieuwke{other example}


==> conclusion.tex <==
\section{Conclusion}


==> data_distributions.tex <==
\section{Data Distribution}
In accordance with the data described in section \ref{lt_data}, we present the distribution of all compositions in the train and various test sets. It can be seen that the test sets \lq heldout\_tables\rq{} and \lq new\_compositions \rq{} are the most difficult and require zero-shot (or one shot??) generalisation owing to their significantly different distribution as compared to \lq train \rq{}.
\begin{figure}[!ht]
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=0.95\linewidth, trim={15mm, 5mm, 35mm, 15mm}, clip]{figures/train}
    \caption{Train}\label{fig:train_dist}
    \end{subfigure}
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=0.95\linewidth, trim={15mm, 5mm, 35mm, 15mm}, clip]{figures/heldout_inputs}
    \caption{Heldout Inputs}\label{fig:held_ipt}
    \end{subfigure}
    \begin{subfigure}{0.45\linewidth}
   	\includegraphics[width=0.95\linewidth, trim={15mm, 5mm, 35mm, 15mm}, clip]{figures/heldout_compositions}
   	\caption{Heldout Compositions}\label{fig:held_comp}
    \end{subfigure}
    \begin{subfigure}{0.45\linewidth}
   	\includegraphics[width=0.95\linewidth, trim={15mm, 5mm, 35mm, 15mm}, clip]{figures/heldout_tables}
   	\caption{Heldout Tables}\label{fig:held_tab}
    \end{subfigure}
    \begin{subfigure}{0.45\linewidth}
   	\includegraphics[width=0.95\linewidth, trim={15mm, 5mm, 35mm, 15mm}, clip]{figures/new_compositions}
   	\caption{New Compositions}\label{fig:new_comp}
    \end{subfigure}
\caption{Data distribution of train and all test sets}\label{fig:all_data}
\end{figure}


==> implementation.tex <==
\subsection{AG loss} 

\comment{describe loss term of AG}
\comment{The loss term \ldots}
% We implement AG by extending a model's loss with an additional term, which captures the difference between the model's computed attention and the target attention pattern that is provided to the model at training time:

\[\mathcal{L}_{\text{AG}} = \frac{1}{T}\left( \sum_{t=1}^T{\sum_{i=1}^N} -a_{i,t} \log\hat{a}_{i,t}\right) \],

where $T$ is the length of the output string, $N$ is the length of the input string, $\hat{a}_{i,t}$ is the decoder-computed attention of input token $i$ at time $t$ and $a_{i,t}$ is its corresponding attention target.
At training time, we weight the original loss of the model and the AG loss with their corresponding weighting factors.

Along with the extra loss term, we introduce also a new \textit{gating} attention mechanism, which we call \textit{full-focus}.
The full-focus attention mechanism is designed to force the decoder to take into account the context vector, by \textit{multiplying} it with the embedded inputs to the decoder, rather than concatenating these two vectors.
\comment{This is not entirely correct I think? @Elia this should be reviewed.}

$$
di_t = c_t(eo, do_{t-1}) \odot ReLU(W_f * [de_t; c_t(eo, do_{t-1})])
$$

A schematic of attentive guidance is given in Figure \ref{fig:attentive_guidance}.
\footnote{Our code and datasets are available at: \url{https://github.com/i-machine-think/machine} and \url{https://github.com/i-machine-think/machine-tasks}, respectively.}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/model}
    \caption{
At each time step $t$, the AG-guided model infers a variable-length alignment weight vector $\hat{a}$ based on the current target state $h_{t}$ and all source states. The Cross Entropy $D$ between $\hat{a}$ and the one-hot AG target $a$ is computed. A context vector $c_{t}$ is then calculated as the weighted average, according to $\hat{a}$ over all the encoder states and is then concatenated with the output of the previous step to generate the next prediction. }\label{fig:attentive_guidance} % Elia
\end{figure*}
%\kris{I would not have the last encoder state pointing to the decoder state directly, but to the input of the decoder. The first decoder has two inputs. One from the last encoder, one from attention}


==> models.tex <==
\subsection{Models}

In our experiments, we test and compare 3 different models
First, we establish baseline, which is a standard encoder-decoder models with an attention mechanism that is learned end-to-end along with the rest of the parameters (\textit{baseline})
The second model is identical from an architectural perspective, but has the additional training objective to minimise the cross-entropy loss between the calculated attention vectors and a provided target attention vectors in its backward pass (\textit{guided}).
To take apart the learnability of the target attention patterns and their effect on the learned solution, we also test the impact of replacing the calculated attention vectors in the forward pass of a model with the target attention vectors (\textit{oracle guidance})

% \kris{
% We test and compare three different models. First we establish a baseline, which is a standard sequence-to-sequence model with a self-learned attention mechanism (\textit{baseline}).
% The second model is the same sequence-to-sequence network, where we replace the calculated attention vectors in the forward pass with the provided one-hot vectors (\textit{oracle guidance}).
% The third model does use the calculated attention vectors in its forward pass, but minimizes the cross-entropy loss between the calculated attention vectors and provided one-hot vectors in its backward pass (\textit{learned guidance}).
% }

For a fair comparison of the models, we perform a modest grid search over multiple parameter set sizes and attention mechanisms. 
We run each configuration 3 times and use the average output sequence loss on a validation set to pick the models. \dieuwke{we actually picked based on heldout tables, not sure if we should put that here as justification in the results comes only way later}.
The resulting configurations are shown in Table \ref{table:train-details}

\begin{table}[!ht]
\centering
\begin{tabular}{|l|l|l|}
\hline
                           & \textbf{Baseline}  & \textbf{Learned guidance} \\ \hline % & \textbf{Hard guidance} \\ \hline
\textbf{RNN cell}          & GRU                & GRU                       \\ \hline % & GRU                    \\ \hline
\textbf{Batch size}        & 64                 & 64                        \\ \hline % & 64                     \\ \hline
\textbf{Optimizer}         & Adam               & Adam                      \\ \hline % & Adam                   \\ \hline
\textbf{LR}                & 0.001              & 0.001                     \\ \hline % & 0.001                  \\ \hline
\textbf{Max gradient norm} & ?                  & ?                         \\ \hline % & ?                      \\ \hline
\textbf{Dropout}           & 0                  & 0                         \\ \hline % & 0                      \\ \hline
\textbf{Initialization}    & Uniform(-0.8, 0.8) & Uniform(-0.8, 0.8)        \\ \hline % & Uniform(-0.8, 0.8)     \\ \hline
\textbf{Embedding size}    & ?                  & ?                         \\ \hline % & ?                      \\ \hline
\textbf{Hidden size}       & ?                  & ?                         \\ \hline % & ?                      \\ \hline
\end{tabular}
\caption{Training details of the selected models}
\label{table:train-details}
\end{table}

